The Tenth NTIRE 2025 Efficient Super-Resolution Challenge Report

This paper presents a comprehensive review of the NTIRE 2025 Challenge on Single-Image Efficient Super-Resolution (ESR). The challenge aimed to advance the development of deep models that optimize key computational metrics, i.e., runtime, parameters, and FLOPs, while achieving a PSNR of at least 26.90 dB on the $\operatorname{DIV2K\_LSDIR\_valid}$ dataset and 26.99 dB on the $\operatorname{DIV2K\_LSDIR\_test}$ dataset. A robust participation saw \textbf{244} registered entrants, with \textbf{43} teams submitting valid entries. This report meticulously analyzes these methods and results, emphasizing groundbreaking advancements in state-of-the-art single-image ESR techniques. The analysis highlights innovative approaches and establishes benchmarks for future research in the field.

==> section/author_helper.tex <==
Bin Ren and
Hang Guo and 
Lei Sun and 
Zongwei Wu and 
Radu Timofte and 
Yawei Li and 
Yao Zhang and
Xinning Chai and
Zhengxue Cheng and 
Yingsheng Qin and
Yucai Yang and
Li Song and 
Hongyuan Yu and 
Pufan Xu and 
Cheng Wan and 
Zhijuan Huang and 
Peng Guo and 
Shuyuan Cui and 
Chenjun Li and 
Xuehai Hu and 
Pan Pan and 
Xin Zhang and 
Heng Zhang and 
Qing Luo and 
Linyan Jiang and 
Haibo Lei and 
Qifang Gao and 
Yaqing Li and 
Weihua Luo and
Tsing Li and
Qing Wang and
Yi Liu and
Yang Wang and
Hongyu An and
Liou Zhang and
Shijie Zhao and
Lianhong Song and
Long Sun and
Jinshan Pan and
Jiangxin Dong and
Jinhui Tang and
Jing Wei and
Mengyang Wang and
Ruilong Guo and
Qian Wang and
Qingliang Liu and
Yang Cheng and
Davinci and
Enxuan Gu and
Pinxin Liu and
Yongsheng Yu and
Hang Hua and
Yunlong Tang and
Shihao Wang and
Yukun Yang and
Zhiyu Zhang and
Yukun Yang and
Jiyu Wu and
Jiancheng Huang and
Yifan Liu and
Yi Huang and
Shifeng Chen and
Rui Chen and
Yi Feng and
Mingxi Li and
Cailu Wan and
Xiangji Wu and
Zibin Liu and
Jinyang Zhong and
Kihwan Yoon and
Ganzorig Gankhuyag and 
Shengyun Zhong and 
Mingyang Wu and 
Renjie Li and 
Yushen Zuo and 
Zhengzhong Tu and 
Zongang Gao and 
Guannan Chen and 
Yuan Tian and 
Wenhui Chen and 
Weijun Yuan and
Zhan Li and
Yihang Chen and
Yifan Deng and
Ruting Deng and
Yilin Zhang and
Huan Zheng and
Yanyan Wei and
Wenxuan Zhao and
Suiyi Zhao and
Fei Wang and
Kun Li and
Yinggan Tang and
Mengjie Su and
Jae-hyeon Lee and
Dong-Hyeop Son and
Ui-Jin Choi and
Tiancheng Shao and
Yuqing Zhang and
Mengcheng Ma and
Donggeun Ko and
Youngsang Kwak and
Jiun Lee and
Jaehwa Kwak and
Yuxuan Jiang and
Qiang Zhu and
Siyue Teng and
Fan Zhang and
Shuyuan Zhu and
Bing Zeng and
David Bull and
Jing Hu and
Hui Deng and
Xuan Zhang and
Lin Zhu and
Qinrui Fan and
Weijian Deng and
Junnan Wu and
Wenqin Deng and
Yuquan Liu and
Zhaohong Xu and
Jameer Babu Pinjari and
Kuldeep Purohit and
Zeyu Xiao and
Zhuoyuan Li and
Surya Vashisth and
Akshay Dudhane and
Praful Hambarde and
Sachin Chaudhary and
Satya Naryan Tazi and
Prashant Patil and
Santosh Kumar Vipparthi and
Subrahmanyam Murala and
Wei-Chen Shen and
I-Hsiang Chen and
Yunzhe Xu and
Chen Zhao and
Zhizhou Chen and
Akram Khatami-Rizi and
Ahmad Mahmoudi-Aznaveh and
Alejandro Merino and
Bruno Longarela and
Javier Abad and
Marcos V. Conde and
Simone Bianco and
Luca Cogo and
Gianmarco Corti


% Some Summary or Comments for Next years Challenge (2026):
1. Ask every team to named their Fig. starts withe team name.
2. Ask each team describe their method as "they" 
3. Ask each team to use Three or Five Key Words to describe their method, then we can do some statistic show in our report
4. The PSNR threshold can be adjust higher next year.
5. Ask each team who want to co-author the report paper, their team update must meets: 
- Method, 
- Training Details,
- Length: between 0.5 to 1 page.

==> teams/affiliation.tex <==
\subsection*{Your team name}
\noindent\textit{\textbf{Title: }} Title of your Paper or Methods\\
\noindent\textit{\textbf{Members: }} \\
Team member 1$^1$ (\href{mailto:yourEmail@xxx.xxx}{yourEmail@xxx.xxx}),\\
Team member 2$^2$, \\
Team member 3$^3$, \\
\noindent\textit{\textbf{Affiliations: }} \\ 
$^1$ Affiliation 1 \\
$^2$ Affiliation 2 \\
$^3$ Affiliation 3 \\



==> teams/team07_NanoSR/affiliation.tex <==
\subsection*{NanoSR}
\noindent\textit{\textbf{Title: }} Title of your Paper or Methods\\
\noindent\textit{\textbf{Members: }} \\
Team member 1$^1$ (\href{mailto:yourEmail@xxx.xxx}{yourEmail@xxx.xxx}),\\
Team member 2$^2$, \\
Team member 3$^3$, \\
\noindent\textit{\textbf{Affiliations: }} \\ 
$^1$ Affiliation 1 \\
$^2$ Affiliation 2 \\
$^3$ Affiliation 3 \\



==> teams/team16_SCMSR/affiliation.tex <==
\subsection*{SCMSR}
\noindent\textit{\textbf{Title: }} Title of your Paper or Methods\\
\noindent\textit{\textbf{Members: }} \\
Team member 1$^1$ (\href{mailto:yourEmail@xxx.xxx}{yourEmail@xxx.xxx}),\\
Team member 2$^2$, \\
Team member 3$^3$, \\
\noindent\textit{\textbf{Affiliations: }} \\ 
$^1$ Affiliation 1 \\
$^2$ Affiliation 2 \\
$^3$ Affiliation 3 \\



==> teams/team16_SCMSR/main.tex <==
\subsection{SCMSR}

==> teams/team33_EagleSR/affiliation.tex <==
\subsection*{EagleSR}
\noindent\textit{\textbf{Title: }} Title of your Paper or Methods\\
\noindent\textit{\textbf{Members: }} \\
Team member 1$^1$ (\href{mailto:yourEmail@xxx.xxx}{yourEmail@xxx.xxx}),\\
Team member 2$^2$, \\
Team member 3$^3$, \\
\noindent\textit{\textbf{Affiliations: }} \\ 
$^1$ Affiliation 1 \\
$^2$ Affiliation 2 \\
$^3$ Affiliation 3 \\



==> teams/team33_EagleSR/main.tex <==
\subsection{EagleSR}

==> teams/team39_MiSR/affiliation.tex <==
\subsection*{MiSR}
\noindent\textit{\textbf{Title: }} Title of your Paper or Methods\\
\noindent\textit{\textbf{Members: }} \\
Team member 1$^1$ (\href{mailto:yourEmail@xxx.xxx}{yourEmail@xxx.xxx}),\\
Team member 2$^2$, \\
Team member 3$^3$, \\
\noindent\textit{\textbf{Affiliations: }} \\ 
$^1$ Affiliation 1 \\
$^2$ Affiliation 2 \\
$^3$ Affiliation 3 \\



==> teams/team39_MiSR/main.tex <==
\subsection{MiSR}

==> teams/team43_SVM/affiliation.tex <==
\subsection*{SVM}
\noindent\textit{\textbf{Title: }} Title of your Paper or Methods\\
\noindent\textit{\textbf{Members: }} \\
Team member 1$^1$ (\href{mailto:yourEmail@xxx.xxx}{yourEmail@xxx.xxx}),\\
Team member 2$^2$, \\
Team member 3$^3$, \\
\noindent\textit{\textbf{Affiliations: }} \\ 
$^1$ Affiliation 1 \\
$^2$ Affiliation 2 \\
$^3$ Affiliation 3 \\



==> teams/team43_SVM/main.tex <==
\subsection{SVM}

==> teams/team46_SRCB/main.tex <==
\subsection{SRCB}

Swift Parameter-free Attention Network (SPAN)~\cite{wan2024swift} has won the first place in The Ninth NTIRE 2024 Efficient Super-Resolution Challenge. So, the team uses it as baseline. They prune the last layer via L2 norm and retrain the model with mixup data augmentation.
